STCOcc: Sparse Spatial-Temporal Cascade Renovation for 3D Occupancy and Scene Flow Prediction

3D occupancy and scene flow offer a detailed and dynamic representation of 3D scene. Recognizing the sparsity and complexity of 3D space, previous vision-centric methods have employed implicit learning-based approaches to model spatial and temporal information. However, these approaches struggle to capture local details and diminish the model's spatial discriminative ability. To address these challenges, we propose a novel explicit state-based modeling method designed to leverage the occupied state to renovate the 3D features. Specifically, we propose a sparse occlusion-aware attention mechanism, integrated with a cascade refinement strategy, which accurately renovates 3D features with the guidance of occupied state information. Additionally, we introduce a novel method for modeling long-term dynamic interactions, which reduces computational costs and preserves spatial information. Compared to the previous state-of-the-art methods, our efficient explicit renovation strategy not only delivers superior performance in terms of RayIoU and mAVE for occupancy and scene flow prediction but also markedly reduces GPU memory usage during training, bringing it down to 8.7GB. Our code is available on https://github.com/lzzzzzm/STCOcc

==> figures/figures-tex/Ablation_OA-SCA_V2.tex <==
\begin{figure}[tp]
    \begin{minipage}{0.3\textwidth}
    \includegraphics[width=5cm]{figures/Ablation_W-O-OA-SCA.pdf}
    \end{minipage}
    \noindent
    \begin{minipage}{0.17\textwidth}
        \centering
        \resizebox{1.0\textwidth}{!}{
        \begin{tabular}{c|c}
           \toprule
           Method  &  RayIoU    \\
           \midrule
           W/O SCA                  & 37.4      \\
           SCA~\cite{bevformer}     & 37.2      \\    
           DA-SCA~\cite{fbbev}      & 37.4       \\  
           \midrule
           OA-SCA                   & \textbf{38.2} \\
           \bottomrule
        \end{tabular}
        }
    \end{minipage}
    \caption{\textbf{Ablation on the OA-SCA module.} We visualize the features after refinement both with and without the OA-SCA module, and further conduct an ablation study comparing the OA-SCA with the SCA and DA-SCA modules proposed in previous methods~\cite{bevformer, fbbev}.}
    \label{label:ablation-oa-sca}
\end{figure}

==> figures/figures-tex/motivation.tex <==
\begin{figure}[t!]
    \centering
    \begin{subfigure}{0.23\textwidth}
        \centering
        \includegraphics[width=0.87\linewidth]{figures/Motivation-Spatial.pdf}
        \caption{Spatial Modeling Comparison.}
        \label{figure:motivation-Spatial-modeling}
    \end{subfigure}
    \centering
    \begin{subfigure}{0.24\textwidth}
        \centering
        \includegraphics[width=0.96\linewidth]{figures/Motivation-temporal.pdf}
        \caption{Temporal Modeling Comparison.}
        \label{figure:motivation-Temporal-modeling}
    \end{subfigure}
    \begin{subfigure}{0.47\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/model_comparsion.pdf}
        \caption{Comparison with Different Models.}
        \label{figure:motivation-model-comparsion}
    \end{subfigure}
    \caption{\textbf{(a) Comparison with Different 3D Spatial Modeling Methods:} Our method addresses the ambiguities found in previous sparse methods while maintaining sparsity. \textbf{(b) Comparison with Different Temporal Modeling Methods:} Our proposed sparse level long-term temporal modeling reduces computation costs while perserving spatial consistency. \textbf{(c) Compared with Other Methods:} Our approach achieves state-of-the-art performance of RayIoU and MAVE with lower training costs.}
    \vspace{-1.5em}
    \label{figure:motivation}
\end{figure}



==> figures/figures-tex/visualize_results.tex <==
\begin{figure*}[t]
    \centering
    \scriptsize
    \setlength\tabcolsep{1pt} % default value: 6pt
    \newcommand{\Figwidth}{0.22\linewidth}
    \begin{tabular}{cccc}
    Ground Truth & Ours & SparseOcc & FBOCC \\
    \includegraphics[trim={50 80 100 80},clip,width=\Figwidth]{figures/images/occ3d-val-29/gt_29.jpg} &
    \includegraphics[trim={50 80 100 80},clip,width=\Figwidth]{figures/images/occ3d-val-29/ours_29.jpg} &
    \includegraphics[trim={50 80 100 80},clip,width=\Figwidth]{figures/images/occ3d-val-29/sparseocc_29.jpg} &
    \includegraphics[trim={50 80 100 80},clip,width=\Figwidth]{figures/images/occ3d-val-29/fbocc_29.jpg} \\
    \includegraphics[trim={50 80 100 80},clip,width=\Figwidth]{figures/images/occ3d-val-1818/gt-1818.jpg} &
    \includegraphics[trim={50 80 100 80},clip,width=\Figwidth]{figures/images/occ3d-val-1818/ours-1818.jpg} &
    \includegraphics[trim={50 80 100 80},clip,width=\Figwidth]{figures/images/occ3d-val-1818/sparseocc-1818.jpg} &
    \includegraphics[trim={50 80 100 80},clip,width=\Figwidth]{figures/images/occ3d-val-1818/fbocc-1818.jpg} \\
    \end{tabular}
	\caption{\textbf{Qualitative results on Occ3d-nus validation set.} Our method produces detailed predictions for objects such as cars and trucks, while also providing clear boundary layouts for structures like buildings and vegetation.}
    \label{figure:visualization}
    \vspace{-0.5cm}
\end{figure*}

==> table/ablation_OA.tex <==
\begin{minipage}{0.5\textwidth}

\begin{minipage}[t]{0.4\textwidth}
    \makeatletter\def\@captype{table}
    \resizebox{0.8\textwidth}{!}{
    \begin{tabular}{ccccc}
        \toprule
        Method    & RayIoU   \\
        \midrule
        W/O SCA    & 37.4    \\
        SCA        & 37.2   \\
        DA-SCA     & 37.4   \\
        \midrule
        OA-SCA     & \textbf{38.2} \\
        \bottomrule
    \end{tabular}
    }
    \caption{\textbf{Ablation on the OA-SCA module.}}
    \label{table:ablation-oa-sca}
\end{minipage}
\begin{minipage}[t]{0.5\textwidth}
    \makeatletter\def\@captype{table}
    \resizebox{0.9\textwidth}{!}{
    \begin{tabular}{ccc}
        \toprule
        Method     & RayIoU     & MAVE         \\
        \midrule
        W/O TSA    &   &     \\   
        TSA        &   &      \\
        \midrule
        OA-TSA     &   &       \\
        \bottomrule
    \end{tabular}
    }
    \caption{\textbf{Ablation on the OA-TSA module.}}
    \label{table:ablation-oa-tsa}
\end{minipage}

\end{minipage}


==> table/mainresults_MAVE_Occ3d.tex <==
\begin{table}[tp]
    \setlength{\tabcolsep}{0.010\linewidth}
    \centering
    \scriptsize
    \label{table:rayiou-occ3d}
  \scalebox{1.0}{
  \begin{tabular}{l|cc|>{\columncolor{Gray}}c}
    \toprule
    Method      & Backbone  & Input Size & MAVE \\
    \midrule
    BEVFormer~\cite{bevformer}      & Intern-Tiny &1600$\times$900 &0.695  \\
    FB-Occ~\cite{fb-occ}            & Intern-Tiny &704$\times$256  &0.433 \\
    ViewFormer~\cite{viewformer}    & Intern-Tiny &704$\times$256  &0.412 \\
    \midrule
    STCOcc      & R50         &704$\times$256  &0.321     \\  
    \bottomrule
  \end{tabular}
  }
  \caption{\textbf{Comparison of MAVE performance on the FlowOcc3D~\cite{viewformer} dataset.}}
\end{table}
